Synchronous Byzantine Lattice Agreement in ${\cal O}(\log (f))$ Rounds

In the Lattice Agreement (LA) problem, originally proposed by Attiya et al. \cite{Attiya:1995}, a set of processes has to decide on a chain of a lattice. More precisely, each correct process proposes an element $e$ of a certain join-semi lattice $L$ and it has to decide on a value that contains $e$. Moreover, any pair $p_i,p_j$ of correct processes has to decide two values $dec_i$ and $dec_j$ that are comparable (e.g., $dec_i \leq dec_j$ or $dec_j < dec_i$). LA has been studied for its practical applications, as example it can be used to implement a snapshot objects \cite{Attiya:1995} or a replicated state machine with commutative operations \cite{Faleiro:2012}. Interestingly, the study of the Byzantine Lattice Agreement started only recently, and it has been mainly devoted to asynchronous systems. The synchronous case has been object of a recent pre-print \cite{Zheng:aa} where Zheng et al. propose an algorithm terminating in ${\cal O}(\sqrt f)$ rounds and tolerating $f < \lceil n/3 \rceil$ Byzantine processes. In this paper we present new contributions for the synchronous case. We investigate the problem in the usual message passing model for a system of $n$ processes with distinct unique IDs. We first prove that, when only authenticated channels are available, the problem cannot be solved if $f=n/3$ or more processes are Byzantine. We then propose a novel algorithm that works in a synchronous system model with signatures (i.e., the {\em authenticated message} model), tolerates up to $f$ byzantine failures (where $f<n/3$) and that terminates in ${\cal O}(\log f)$ rounds. We discuss how to remove authenticated messages at the price of algorithm resiliency ($f < n/4$). Finally, we present a transformer that converts any synchronous LA algorithm to an algorithm for synchronous Generalised Lattice Agreement.

==> bibliography.tex <==
\begin{thebibliography}{10}

\bibitem{andoSY95}
H.~Ando, I.~Suzuki, and M.~Yamashita.
\newblock Formation and agreement problems for synchronous mobile robots with
  limited visibility.
\newblock In {\em Proc. of the 10th  IEEE Symp. on Intelligent Control}, pages
  453--460, 1995.
  
  
%\bibitem{BeMB13}
%M. Beinhofer, J. Muller, and W. Burgard.
%Effective landmark placement for accurate and reliable mobile robot navigation.
%\newblock {\em Robotics and Autonomous Systems}, 
% 61(10):  1060--1069, 2013.
  
% \bibitem{BhGM16}
% S. Bhagat, S. Gan Chaudhuri, and K. Mukhopadhyaya.
% \newblock Formation of general position by asynchronous mobile robots 
% under one-axis agreement
%\newblock In {\em Proc. of the  10th International Workshop on Algorithms and Computation
%(WALCOM)}, pages  80--91, 2016.

 \bibitem{BrT16}
Q. Bramas and  S. Tixeuil.
Brief announcement: Probabilistic asynchronous arbitrary pattern formation.
\newblock In {\em Proc.  of the 34th ACM Symposium on Principles of Distributed Computing
(PODC)},  pages 443--445,
 {2016}.



  \bibitem{CiDN16}
   S. Cicerone, G. Di Stefano, and A.  Navarra.
\newblock  Asynchronous embedded pattern formation without orientation.
\newblock In {\em Proc. of the 30th International Symposium on Distributed Computing
(DISC)}, pages 85--98, 2016.

%  \bibitem{CiDN18}
%   S. Cicerone, G. Di Stefano, and A.  Navarra.    
% \newblock  Gathering of robots on meeting-points: feasibility and optimal resolution algorithms.
% \newblock   {\em Distributed Computing} 31(1): 1--50, 2018.


%\bibitem{DaFPSY16}
%S.~Das, P.~Flocchini, G.~Prencipe, N.~Santoro, and M.~Yamashita.
%\newblock Autonomous mobile robots with lights.
%\newblock {\em Theoretical Computer Science}, 609(P1):171--184, January 2016.

\bibitem{DaFSY15}
S.~Das, P.~Flocchini, N.~Santoro, and M.~Yamashita.
\newblock Forming sequences of geometric patterns with oblivious mobile robots.
\newblock {\em Distributed Computing}, 28(2):131--145, April 2015.


\bibitem{DiFlSVY17}
G.~{Di Luna}, P.~Flocchini, N.~Santoro, G.~Viglietta, and M.~Yamashita.
\newblock Meeting in a polygon by anonymous oblivious robots.
\newblock In {\em Proc. of the 31st International Symposium on Distributed Computing
(DISC)}, pages 14:1-14:15, 2017.

%\bibitem{DeFN16}
%M.~D'Emidio, D.~Frigioni, and A.~Navarra.
%\newblock Synchronous robots vs asynchronous lights-enhanced robots on graphs.
%\newblock {\em Elec. Notes Th. Comp. Sci.}, 322:169--180, 2016.


\bibitem{ErRS13}
M.  Erdelj, T. Razafindralambo, and D. Simplot-Ryl.
Covering points of interest with mobile sensors.
\newblock {\em IEEE Transactions on Parallel and Distributed Systems} 24(1):32--43, 2013.
	
\bibitem{FloPS12}
P.~Flocchini, G.~Prencipe, and N.~Santoro.
\newblock {\em Distributed Computing by Oblivious Mobile Robots}.
\newblock Morgan \&
  Claypool, 2012.

\bibitem{FPSW08}
P.~Flocchini, G.~Prencipe, N.~Santoro, and P.~Widmayer.
\newblock Arbitrary pattern formation by asynchronous oblivious robots.
\newblock {\em Theoretical Computer Science}, 407(1-3):412--447, 2008.

\bibitem{FloSVY16}
P.~Flocchini, N.~Santoro, G.~Viglietta, and M.~Yamashita.
\newblock Rendezvous with constant memory.
\newblock {\em Theoretical Computer Science}, 621:57--72, 2016.

%\bibitem{Fujinaga10}
%Fujinaga N., Ono H., Kijima S., Yamashita M. (2010) Pattern Formation through Optimum Matching by Oblivious CORDA Robots. In Proc: Principles of Distributed Systems (OPODIS 2010). Lecture Notes in Computer Science, vol 6490. Pages 1--15, 2010.

\bibitem{FuYOKY15}
N.~Fujinaga, Y.~Yamauchi, H. Ono, S.~Kijima, and M.~Yamashita.
\newblock Pattern formation by oblivious asynchronous mobile robots. 
\newblock {\em SIAM Journal on Computing}, 44(3):740--785, 2015.

\bibitem{FuYaKiYa12}
N.~Fujinaga, Y.~Yamauchi, S.~Kijima, and M.~Yamashita.
\newblock Asynchronous pattern formation by anonymous oblivious mobile robots.
\newblock  In {\em Proc. of the 26th International Symposium on Distributed Computing
(DISC)}, pages 312--325, 2012.

%\bibitem{patrolling13} A. Collins, J. Czyzowicz, L. Gąsieniec, A. Kosowski, E. Kranakis, D. Krizanc,
%R. Martin, and O. Morales Ponce. Optimal Patrolling of Fragmented Boundaries.
%In Proceedings of the Twenty-fifth Annual ACM Symposium on Parallelism in Algorithms and Architectures (SPAA ’13), pages 241–250, New York, USA, 2013.
%
%\bibitem{patrolfaulty} J. Czyzowicz, L. Gąsieniec, A. Kosowski, E. Kranakis, D. Krizanc, and N. Taleb.
%When Patrolmen Become Corrupted: Monitoring a Graph using Faulty Mobile
%Robots In Proc. ISAAC 2015, 26th International Symposium on Algorithms and
%Computation, pages 343-354, 2015.

\bibitem{collisionfree}
R. Guerraoui and A. Maurer.
Collision-Free Pattern Formation. 
 In {\em Proc. of the 20th International Conference on Principles of Distributed Systems (OPODIS)}, pages 16:1-16:13, 2016.

%\bibitem{ShBM15}
%G.~Sharma, C.~Busch, and S.~Mukhopadhyay.
%\newblock Mutual visibility with an optimal number of colors.
%\newblock In {\em 11th International Symposium on Algorithms and Experiments
%  for Wireless Sensor Networks (Algosensors)}, pages 196--201, 2015.

\bibitem{SugS96}
K.~Sugihara and I.~Suzuki.
\newblock Distributed algorithms for formation of geometric patterns with many
  mobile robots.
\newblock {\em Journal of Robotics Systems}, 13:127--139, 1996.


\bibitem{SuzY99}
I.~Suzuki and M.~Yamashita.
\newblock Distributed anonymous mobile robots: Formation of geometric patterns.
\newblock {\em SIAM Journal on Computing}, 28(4):1347--1363, 1999.

\bibitem{yamashita2010}
M.~Yamashita and I.~Suzuki.
\newblock Characterizing geometric patterns formable by oblivious anonymous
  mobile robots.
\newblock {\em Theoretical Computer Science}, 411(26-28):2433--2453, 2010.

\bibitem{YuY14}
Y. Yamauchi and M. Yamashita.
\newblock    Randomized pattern formation algorithm for asynchronous oblivious mobile robots.
In {\em Proc. of the 28th International Symposium on Distributed Computing (DISC)}, pages 137--151, 2014.


\end{thebibliography}


==> macros.tex <==
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}
% Used for displaying a sample figure. If possible, figure files should
% be included in EPS format.
%
% If you use the hyperref package, please uncomment the following line
% to display URLs in blue roman font according to Springer's eBook style:
% \renewcommand\UrlFont{\color{blue}\rmfamily}
\newtheorem{observation}{Observation}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{Lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newcommand{\moveall}{{\sc Move-All}\xspace}
\newcommand{\permute}{Permute\xspace}

\newcommand{\visitall}{{\sc Visit-All}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Comment management
\newif\ifshowcomments
\showcommentstrue
% \showcommentsfalse

\ifshowcomments
\newcommand{\mynote}[2]{\fbox{\bfseries\sffamily\scriptsize{#1}}
 {\small$\blacktriangleright$\textsf{\emph{#2}}$\blacktriangleleft$}}
\else
\newcommand{\mynote}[2]{}
\fi
\newcommand{\giuseppe}[1]{\textcolor{olive}{\mynote{GADL}{#1}}}
\newcommand{\emmanuelle}[1]{\textcolor{pink}{\mynote{EA}{#1}}}
\newcommand{\silvia}[1]{\textcolor{orange}{\mynote{SB}{#1}}}
\newcommand{\leo}[1]{\textcolor{blue}{\mynote{LQ}{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
